Conservative dielectric functions and electrical conductivities from the multicomponent Bhatnagar-Gross-Krook equation

A considerable number of semi-empirical and first-principles models have been created to describe the dynamic response of a collisionally damped charged-particle system. However, known challenges persist for established dynamic structure factors (DSF), dielectric functions, and conductivities. For instance, the semi-empirical Drude-Smith conductivity [N.M. Smith, Phys. Rev. B 64, 155106 (2001)] lacks interpretability, and the first-principles Mermin dielectric function [N.D. Mermin, Phys. Rev. B, 1, 2362 (1970)] does not satisfy the frequency sum rule [G.S. Atwal and N.W. Ashcroft, Phys. Rev. B 65, 115109 (2002)]. In this work, starting from the multicomponent Bhatnagar-Gross-Krook (BGK) kinetic equation, we produce a multi-species susceptibility that conserves number and momentum, which we refer to as the ``completed Mermin'' susceptibility, and we explore its properties and uses. We show that the completed Mermin susceptibility satisfies the frequency sum (f-sum) rule. We compute the associated DSF and find that momentum conservation qualitatively impacts the DSF's shape for a carbon-contaminated deuterium and tritium plasma under NIF hot-spot conditions. In the appendices, we provide numerical implementations of the completed Mermin susceptibility, for the reader's convenience. Further, we produce a new non-Drude conductivity model, by taking the single-species limit and introducing free parameters in the terms that enforce number and momentum conservation. To illustrate how number and momentum conservation impact the dynamical conductivity shape, we apply our conductivity model to dynamical gold conductivity measurements [Z. Chen, et al., Nature communications, 12.1, 1638, (2021)]. Finally, comparing our model to the Drude-Smith conductivity model, we conclude that Smith's phenomenological parameter violates local number conservation.

==> textstorage.tex <==
%% Multispecies RPA derivation

To derive the Lindhard/RM susceptibilities, start from the zeroth order version of \eqref{eq_kineticf1-multispecies} and introduce the mean field correction via the multispecies Hartree potential,
\begin{align}\label{def_msHartree}
    U_\mathrm{ind} = \sum_j v_{ij}(k) \: \delta n_j(\k,\omega).
\end{align}
The end result is,
\begin{align}
    \delta f_i = \frac{m_i^{-1}\k\cdot \nabla_\v \fML{i} }{\v \cdot \k - \omega_\tau}  \left( U_\mathrm{ext} + \sum_j v_{ij}(k) \delta n_j \right).
\end{align}
We limit our derivation to 2 species, integrate over velocity, do a little algebra, and convert to matrices.
The coupled system of kinetic equations is,
\begin{widetext}
\begin{align}
    \left(
    \begin{bmatrix}
        \varepsilon_1 & 0
        \\ 0 & \varepsilon_2
    \end{bmatrix}
    - v_{12}(k)
    \begin{bmatrix}
        0 & C^M_{1,0} 
        \\ C^M_{2,0} & 0
    \end{bmatrix}    
    \right)
    \begin{bmatrix}
        \delta n_1 
        \\ \delta n_2
    \end{bmatrix} 
    = U_\mathrm{ext}
    \begin{bmatrix}
        C^M_{1,0}
        \\ C^M_{2,0}
    \end{bmatrix}  .
\end{align}
\end{widetext}
In this equation we have grouped  $\varepsilon_i = 1 - v_{ii}(k) C^M_{0,i}$, which is the single species Lindhard dielectric function.
The solution to this 2x2 system of equations is,
\begin{subequations} 
\label{eq_multispeciesV}
\begin{align}
%    \chi_{V,1}(\k,\omega) &=  \frac{C^M_{1,0}\left( d_2 + v(k) Z_1 Z_2 C_{2,0}^M \right)}{d_1 d_2 - (Z_1^2 v(k) C^M_{1,0}) \left( Z_2^2 v(k) C^M_{2,0}\right) }
    \chi_{RM,1}(\k,\omega) &=  \frac{C^M_{1,0}\left( \varepsilon_2 + v_{12}(k) C^M_{2,0} \right)}{\varepsilon_1 \varepsilon_2 -  v^2_{12}(k) C^M_{1,0} C^M_{2,0} },
    \\ \chi_{RM,2}(\k,\omega) &= \frac{C^M_{2,0}\left( \varepsilon_1 + v_{12}(k) C^M_{1,0} \right)}{\varepsilon_1 \varepsilon_2 - v^2_{12}(k) C^M_{1,0} C^M_{2,0} } .
\end{align}
\end{subequations}
Recognize these are expressions are for the density-density susceptibility given in \eqref{def_density-densitysuscept}. 
Each term from the sum can be identified:
\begin{subequations} 
\begin{align}
    \chi_{RM,11}(\k,\omega) &=  \frac{C^M_{1,0} \varepsilon_2 }{\varepsilon_1 \varepsilon_2 - v_{12}(k)^2 C^M_{1,0} C^M_{2,0} },
    \\ \chi_{RM,12}(\k,\omega) &=  \frac{ v_{12}(k) C^M_{1,0} C^M_{2,0} }{\varepsilon_1 \varepsilon_2 - v^2_{12}(k) C^M_{1,0} C^M_{2,0} }.
\end{align}
\end{subequations}
It is comforting to note, that this limiting case matches the RPA expression derived in Selchow et at. \cite{Selchow2001DSF}. 

Furthermore, the typical single species $\chi_{V,1} = C^M_{1,0} / \varepsilon_1$, arises by dropping the mean field coupling term. 


\subsection{Dispersion relations}
The list of the multispecies susceptibilities derived so far is: multispecies Lindhard/RM susceptibility \eqref{eq_multispeciesV}, Mermin susceptibility \eqref{eq_multispeciesmermin}, and completed Mermin susceptibility \eqref{eq_multispeciesCM}.

Unlike the single species section there is no tabulation of the energy loss function expansions.
These expansions become incredibly large and intractable.
Instead, we choose to study the dispersion relations and sum rules using the more typical pole expansion \cite{Ropke1998, Selchow1999, Selchow2001DSF, selchow2002extended},
\begin{align}
     \text{Im} \{ \varepsilon^{-1}_i \} = - \pi \sum_n \Big \vert \frac{\partial }{\partial \omega } \text{Re} \{ \varepsilon_i \} \Big \vert_{\omega = \omega_n}^{-1} \delta(\omega - \omega_n),
\end{align}
Expanding the Lindhard/RM, Mermin, and completed Mermin dielectric functions in the high frequency $\omega \rightarrow \infty$ limit, produces,
\begin{align}
    \underset{\omega \rightarrow \infty}{\lim} \varepsilon_i = 1 - \frac{\omega_{p,i}^2}{\omega^2}, 
\end{align}
for all cases. 
About the plasmon poles this expression becomes,
\begin{align} \label{eq_poleexpansion}
    \text{Im} \{ \varepsilon^{-1}_i \} = -\frac{\pi}{2} \omega_{p,i} \left( \delta(\omega - \omega_{p,i}) + \delta(\omega + \omega_{p,i}) \right).
\end{align}
These delta functions would imply that the dispersion relations are all exact.
However, this argument does not hold in the finite $\omega$, $\tau$ limit.

\subsubsection{Sum rules}
The frequency sum (fsum) rule is defined the same as for the single species, \eqref{def_fsumrule-eps}.
However, the perfect screening sum rule changes for the multi-component plasma.
It is,
\begin{align}
    \underset{k \rightarrow 0}{\lim}\: \frac{Z_i \left(\sum_j Z_j \right)}{Z_i^2} \int_{-\infty}^{\infty}  \frac{ d\omega}{ \omega } \text{Im} \{ \varepsilon^{-1} \} = -\pi.
\end{align}
which is consistent with the single species limit \eqref{def_screeningsumrule-eps}.
Using the pole expansion, \eqref{eq_poleexpansion}, implies that both sum rules are satisfied exactly.
However, since these calculations do not hold in the finite $\omega$ limit, multispecies sum rules are studied numerically for finite $\omega$ in the next section.

%% STANTONN MURILLO MODEL
We assume the Stanton and Murillo \cite{StantonMurillo2016} definition of the screening length $\lambda_s$.
\begin{subequations}
\begin{align}
    \lambda_s &= \left( \frac{1}{\lambda_e^2} + \sum_i \frac{1}{\lambda_i^2 (1 + 3 \Gamma_i^{IS}) } \right).
    \\ \lambda_e^{-2} &\approx \frac{4 \pi e^2 n_e}{ \sqrt{T^2 + (\frac{2}{3}E_F)^2}}
    \\ \lambda_i^{-2} &\approx \frac{4 \pi Z_i^2 e^2 n_i}{T}
\end{align} 
\end{subequations}
Where the dimensionless coupling parameter, $\Gamma^{IS}_i$, is defined as
\begin{align}
    \Gamma^{IS}_i &= \frac{e^2}{ a_i T }
\end{align}
and denotes the ratio of an average potential energy and an average kinetic energy.
Here we define the interatomic spacing $a_i$ as,
\begin{align}
    a_i &= \left( \frac{3 Z_i}{ 4 \pi n_e} \right)^{1/3},
    \\ n_e &= \sum_i Z_i n_i
\end{align} 
These relations are obtained by enforcing an overall volumetric constraint $\sum n_i V_i = 1$  where $V_i = 4 \pi a_i^3 /3$ and allotting each ion sphere a volume proportionate to its charge $V_i/Z_i = V_j /Z_j$.


% Non-dimensional susceptibility%
Now consider the susceptibility's factor $n_i/T$.
The factor cancels dimensions with $v(k)$,
\begin{align}
    v(k) \chi_i = \psi_i^2 \left( \frac{1}{\tilde{k}^2 + \tilde{\kappa}^2 } \right) \tilde{\chi},
\end{align}
The factor of $n_i/T$ also cancels dimensions in the full susceptibility equation,
\begin{align}
    \delta \tilde{n}_i = \tilde{\chi} \: \tilde{U}.
\end{align} 
Here $\delta \tilde{n}_i = \delta n_i /n_i$ and $\tilde{U} = U/T$. 


% Sum Rules and FDT 
\section{Sum Rules and the Fluctuation-Dissipation Theorem \label{app_sumrulesFDT}}
Starting from 
\begin{align}
    \int_{-\infty}^{\infty} d\omega \: \omega \text{Im} \{ \varepsilon^{-1} \} = - \pi \omega_p^2 \frac{n}{T} \langle Z \rangle^2 v(k) \frac{k^2}{k_D^2}.
\end{align}
Here the sum rWe can the sum rules in terms of dielectric function using \eqref{def_fsumrule-eps}.
and the ion Debye wavenumber,
\begin{align}
    k_{D,i} &= \sqrt{\frac{4 \pi n_i \langle Z_i \rangle^2 e^2}{T}} = \langle Z_i \rangle \psi_i k_{D,e}.
    \\ \omega_{p,i} &= \sqrt{\frac{4 \pi n_i \langle Z_i \rangle^2 e^2 }{m_i}} = \langle Z_i \rangle \frac{\psi_i}{\zeta_i} \omega_{p,e}.
\end{align} 


The f-sum rule is,
\begin{align}
    - \pi&= \frac{\zeta_i^2}{\psi_i^2} \left(\frac{\tilde{k}^2 + \tilde{\kappa}^2}{\langle Z \rangle^2 \tilde{k}^2} \right) \int_{-\infty}^{\infty} d \tilde{\omega} \: \tilde{\omega} \text{Im}\{ \varepsilon^{-1} \}.
\end{align}
The ``perfect screening'' sum rule \eqref{def_screeningsumrule-eps} is expressed without dimensions.

%\begin{align}
    %\\ & \underset{k \rightarrow 0}{\lim} - \pi \frac{n}{T} v(k) \int \frac{d \tilde{\omega}}{2 \pi}  \: S(k,\omega)
    %\\ &\underset{k \rightarrow 0}{\lim} - \pi \frac{S(k)}{\tilde{k}^2}
    %-\pi &= \underset{k \rightarrow 0}{\lim} \int_{-\infty}^{\infty} d \tilde{\omega} \: \frac{1}{\tilde{\omega}} \ELF 
%\end{align}

The classical Fluctuation-Dissipation Theorem (FDT) is given by,
\begin{align}
    S(k,\omega) = -\frac{2T}{n_i (\omega / \omega_{p,i})} \chi''(k,\omega).
\end{align}
As seen, $\chi$ carries a factor of $n_i/T$ which will cancel with the $T/n_i$ prefactor in the FDT.
This leaves just the $\omega$ which is normalized by $\omega_{p,i}$.
we change the normalization to $\omega_{p,e}$ Which produces, 
\begin{align}\label{eq_FDT-app}
    S(k,\omega) = - 2 \langle Z_i \rangle \frac{\psi_i }{\tilde{\omega} \zeta_i} \tilde{\chi}''(k,\omega).
\end{align}
%We can use the dimensionalized FDT, \eqref{eq_FDT-app} to rewrite the f-sum rule, \eqref{def_fsumrule-Skw}, as,
%\begin{align} 
    %\int \frac{d\omega}{\omega_{p,i}} \frac{1}{2\pi} \left(\frac{\omega}{\omega_{p,i}} \right)^2  S \left(\frac{\omega}{\omega_{p,i},\frac{k}{k_{D,i}}}\right) &= \frac{k a_i}{3 \Gamma_i }
%    \tilde{k}^2 &= - \frac{\zeta_i^2}{\pi} \int_{-\infty}^{\infty} d \tilde{\omega} \: \tilde{\omega} \tilde{\chi}_0'', % = \psi_i^2 \frac{\zeta_i^3}{\psi_i^3} \int \frac{ d \tilde{\omega}}{2 \pi} \: \tilde{\omega}^2  S \left(\tilde{\omega}, \tilde{k} \right) 
%\end{align}

%\todo[inline]{Some of your equations look terrible. I went through to figure out what the $\LaTeX$ issue is. You are variously using different equation environments, often using the array when you only have one equation, which flattens the equation and adds extra white space for no good reason. You might scan the document to ensure that the most appropriate environment is being used. I use `align` unless I have reason to use something else, since it handles both cases (one equation or more) well.}



%OLD contaminated table

\begin{ruledtabular}
\begin{tabular}{c|c c c c c c}
           & n (1/cc) & $\langle Z \rangle$ & $\Gamma$ & $\tilde{\kappa}$ & $\nu_{LL}$ (1/s) & $\nu_{LC}$ (1/s)
\\\hline 1 C pp 200 & 2.33e+26 & 0.965 & 0.145 & 1.196 & 6.05e-03 & 1.51e-04
      \\ 1 C pp 100 & 2.28e+26 & 0.965 & 0.144 & 1.207 & 5.87e-03 & 2.92e-04
      \\ 1 C pp 50 & 2.18e+26 & 0.965 & 0.142 & 1.223 & 5.56e-03 & 5.49e-04
\end{tabular}
\end{ruledtabular}


\section{Introduction \label{sec_intro}}
A considerable amount of work has focused on dynamic response in systems of collisionally damped charged particles, yet challenges persist and there is still demand for accurate estimates of the dynamic structure factor (DSF), dielectric function, and conductivity. The demand comes from many sources, but only a small subset is mentioned here. One source of demand is X-ray Thompson scattering (XRTS) diagnostics, which uses a DSF model to infer plasma properties (i.e. number density, temperature, and ionization) from the scattered x-ray signal [Glenzer and Redmer. Rev. of Modern Phys 81.4 (2009)]. 
Another source of demand comes from experimental efforts to measure the DC conductivity \cite{Celliers2018}.
These experiments use dynamical conductivity models to extrapolate a material's DC conductivity from optical conductivity measurements.
A third source of demand is radiation-hydrodynamics (rad-hydro) codes which use dielectric models to estimate Bremsstrahlung emissions rates [Bachmann et al., PRE 101, 033205 (2020)] and stopping power [Phys. Plasmas 26, 062701 (2019)]. Matching rad-hydro codes to observed emission spectrum allows scientists to quantify the impacts of radiative loss on fusion energy production [Pak et al., PRL 124, 145001 (2020) and Gao et al., PRL 128.18 (2022)]. 
The final source of demand we list is in magnetized linear inertial fusion (MagLIF) experiments which use the Velocity Interferometer System for Any Reflector (VISAR) system [Hemsing, Rev. Sci. Instrum. 50, 73 (1979)] and magnetohydrodynamic (MHD) simulations to “unfold” the time-dependent pressure. In this unfolding process, a MHD code estimates a conductive flyer plate’s response to magnetic pressure and these estimates are matched to the VISAR system’s observation [Hess, et al. High Power Laser Science and Engineering 3 (2015)]. The response is particularly sensitive to conductivity [Cochrane et al. J. Appl. Phys. 119, 105902 (2016)]. Thus, MHD codes equipped with accurate conductivity models can be used with the VISAR system to determine the delivered load current.
% ---- Additional material on the DSF ---- %
%In inertial confinement fusion (ICF) experiments, ablator material is injected into the hot spot from the Rayleigh-Taylor growth of capsule surface perturbations \cite{weber2020mixing}.
%Hot electrons experience Bremstralung radiation more frequently with the high Z material than deuterium or tritium \cite{Bachmann2020}.
%The photons then escape, lowering the hot spot's temperature.
%This radiative loss has been the primary source of variations in observed fusion energy production \cite{Pak2020}.

There are many ways to estimate dynamical response; an emergent method is time-dependent density functional theory (TD-DFT). However, TD-DFT simulations are currently too expensive to satisfy the demand for dynamical response information. Instead, scientists typically use models of dynamical response. Semi-empirical models have free parameters which are tuned to match data. Alternatively, “first principles” models have a functional form that was derived from governing equations and its parameters are computed rather than tuned (often computed from “first principles simulations” like DFT).

Semi-empirical models can lack clear interpretations and require labor intensive fitting procedures. The labor intensity is exemplified by Cochrane et al. [Cochrane et al. J. Appl. Phys. 119, 105902 (2016)] who fit the Lee-More-Desjairlais semi-empirical conductivity model [Contrib. Plasma Phys. 41, 267 (2001)] to DFT estimates and iteratively improved via comparing predictions to experimental measurements. The lack of clear interpretations is exemplified by the non-Drude conductivity models. Both high energy density (HED) and nanomaterials scientists have begun exploring alternatives to the dynamic Drude conductivity model [Hughes and Jeon J Infrared Milli Terahz Waves 33 (2012)] [Kuzel and Nemec. Adv. Optical Mat. 8.3 (2020)]. The primary alternative is the Drude-Smith conductivity model [Phys. Rev. B 64, 155106 (2001)], but Smith’s model has a phenomenological parameter of unknown meaning. [Nemec et al., PRB 79, 115309 (2009) and Crocker et al., PRB 96, 205439 (2017)]. Regardless of whether Smith's parameter is well defined, Terahertz (THz) probes have exposed that fitting the Drude-Smith model to dynamical conductivity and extrapolating a DC conductivity is difficult [Chen et al. Nat Commun 12, 1638 (2021)]. Thus, there is a clear need for interpretable conductivity models which can describe observed non-Drude conductivity behavior.

First principles models have clearer interpretations. The interpretability is exemplified by Mermin’s collision corrected RPA dielectric function [Phys. Rev. B 1, 2362 (1970)], which is built from expanding a kinetic equation with a relaxation model of collisions and enforcing local number conservation (i.e. continuity equation). Mermin’s model requires a dynamical estimate of the species’ collision frequency and research has focused on how we estimate these collision frequencies [Plagemann et al., New Journal of Physics 14.5 (2012), Sperling et al., PRL 115, 115001 (2015), Witte et al., PRL 118, 225001 (2017) and Hentschel et al., Phys. Plasmas 30, 062703 (2023)]. independent of the choice of collision frequency, the Mermin model predicts unphysical behavior. But due to its clear interpretability many works have tied the Mermin model’s unphysical behavior to the fact that it does not include momentum conservation. One example is, Atwal and Ashcroft [Phys. Rev. B 65, 115109 (2002)] which show that Mermin’s number conservation alone cannot produce an infinitesimal plasmon width and thus does not satisfy the correct frequency sum rule. Further, they show that the inclusion of momentum and energy conservation corrects this. Work by Morawetz and Fuhrmann [Phys. Rev. E 62, 4382 (2000)] establishes that Mermin’s dielectric function breaks down in the high frequency limit, but the inclusion of momentum conservation corrects this. However, both works demonstrate that any single species dielectric function which conserves momentum must predict an infinite conductivity. This implies that only multi-species dielectric functions can conserve momentum (therefore satisfy the frequency sum rule) without unphysical conductivity predictions. Currently, multispecies Mermin dielectric functions exist [Selchow et al. Phys. Rev. E 64, 056410 (2001) and Selchow et al. Contributions to Plasma Physics 42.1 (2002)], but they have not been extended to include momentum conservation.

In this work, we produce the first number and momentum conserving multi-species dielectric function from Haack et al.’s multi-species BGK kinetic equation [J Stat. Phys., 168, 826-856 (2017)], which we call the completed Mermin dielectric function. A kinetic equation in the relaxation-time approximation is the typical description used for systems of collisionally damped charged particles. In such an description, the distribution function relaxes to an equilibrium distribution function characterized by local perturbations in the chemical potential, velocity, and temperature. These perturbations are constrained by collisional invariants [Phys. Rev. E 61, 2272 (1999)] which can enforce number, momentum, and energy conservation. Work has been done to connect single species kinetic equations with local perturbations to more established classical kinetic equations. Selchow and Morawetz [PRE 59, 1015 (1999)] derive the Mermin dielectric function [Phys. Rev. B 1, 2362 (1970)] from the classical Fokker-Plank and Bhatnagar, Gross, and Krook’s (BGK) local relaxation kinetic equation [Bhatnagar, Gross, and Krook, Phys. Rev. 94, 511 (1954)]. Atwal and Ashcroft [Phys. Rev. B 65, 115109 (2002)] derive their classical number, momentum, and energy conserving dielectric functions from the BGK kinetic equation. In this study, we connect existing multi-species Mermin-like dynamical response functions [Selchow et al. Phys. Rev. E 64, 056410 (2001)][Selchow et al. Contributions to Plasma Physics 42.1 (2002)], to Haack et al.’s multi-species BGK kinetic equation [J Stat. Phys., 168, 826-856 (2017)]. Connecting these dielectric functions to the BGK kinetic equations affirms our derived completed Mermin dielectric function.

In this work, we find an application of the single species limit of the completed Mermin dielectric function. This dielectric function completes the set of conservative single species dielectric functions: Mermin’s conserves number, our completed Mermin conserves both number and momentum, and Atwal and Ashcroft’s dielectric function conserves number, momentum, and energy. From this set, we can see the impact of each subsequent conservation law. We compare this collection to the dielectric function predicted by Smith’s phenomenological conductivity model and determine that Smith's parameter expresses the extent which number conservation is violated. Additionally, this collection provides alternative first principal conductivity models with interpretable parameters for when non-Drude behavior is observed.


% SAMPLE CONCLUSIONS
%Historically, Lindhard \cite{Lindhard1954} computed the susceptibility of a collisionless electron gas in the solid state regime.
%Lindhard's computation assumed a global relaxation model (RM) for collisions, but let the relaxation time go to infinity.
%Leaving the relaxation time finite could include collisions into the susceptibility, but the global relaxation term did not conserve local number, momentum, and energy \cite{Gross1951, BGK1954}.
%Conservative corrections to Lindhard's susceptibility at finite collision times emerged sporadically and disconnected \cite{Mermin1970, Morawetz2000b, Atwal2002}.
%Some work has already been done to answer this question.
%Selchow et al's work \cite{Selchow1999} showed that both the BGK kinetic equation and the Fokker-Plank kinetic equation produce a Mermin dielectric function.
%Additionally, Morawetz and Fuhrmann's \cite{Morawetz2000b} included momentum conservation via local field corrections; their correction exactly matches the momentum conservation correction in the completed Mermin \eqref{def_chiCM}.
%Morawetz and Fuhrmann notice that the same momentum conservation correction appears regardless of whether you are conserving number and momentum or number, momentum, and energy. 
%Within their local field correction framework, Morawetz and Fuhrmann offer no explanation why the term is unchanged by including of energy conservation.
%However, Our framework anticipates this from the structure of Atwal-Ashcroft's constraint equations \eqref{eq_AAconservationconstraints}.
%The momentum conservation constraint is not coupled to either number density or energy conservation constraints.
%Therefore, we view the inclusion of momentum conservation as the completion of Mermin's original derivation.

% ---- Additional material on the DSF ---- %
%In inertial confinement fusion (ICF) experiments, ablator material is injected into the hot spot from the Rayleigh-Taylor growth of capsule surface perturbations \cite{weber2020mixing}.
%Hot electrons experience Bremstralung radiation more frequently with the high Z material than deuterium or tritium \cite{Bachmann2020}.
%The photons then escape, lowering the hot spot's temperature.
%This radiative loss has been the primary source of variations in observed fusion energy production \cite{Pak2020}.

% Additional material on the VISAR system
%function,the ``unfolding'' procedure which use the Velocity Interferometer System for Any Reflector (VISAR) system \cite{hemsing1979velocity} and magnetohydrodynamic (MHD) simulations to estimate the delivered load current in a magnetized linear inertial fusion (MagLIF) experiment \cite{hess2015efficient}.
%a conductive flyer plate’s response to magnetic pressure and these estimates are matched to the VISAR system’s observation \cite{hess2015efficient}. 
%The estimates are particularly sensitive to conductivity model \cite{cochrane2016magnetically}. 
%Thus, MHD codes equipped with accurate conductivity models can be used with the VISAR system to determine the delivered load current.



% CONCLUSIONS!!!

In this work, we produced a new first principles models of dynamical response models to meet demand in XRTS diagnostics, experimental/theoretical conductivity estimates, and rad hydro codes.
We call this model the completed Mermin susceptibility; it is the first multi-species susceptibility that conserves number and momentum locally.
Our multi-species completed Mermin susceptibility extends the known multi-species Mermin susceptibility.

Furthermore, the single species limit of our completed Mermin model provides a first principles alternative to the semi-empirical Drude-Smith conductivity model.
By comparing the two models, we create a new interpretation of the semi-empirical Drude-Smith conductivity model.
We showed that the Drude-Smith model suppresses DC conductivity by violating local number conservation.
This is contrary to Smith's own argument which claimed $\beta_1$ included back scattering.

We showed numerical and analytic calculations of the f-sum rule and screening sum rule for our completed Mermin.
We argued that Mermin's f-sum rule violation occurs because his continuity equation does not assume $\delta \j = n_0 \delta \u$.
Comparatively, the momentum collisional invariant enforces this assumption.
In the single species limit, our momentum conservation correction matches the local field correction derived in Morawetz and Fuhrmann \cite{Morawetz2000b}.
This momentum conservation correction manifests as an infinitesimal plasmon peak, in the long wavelength limit, which informs us that plasmons are the only energy loss mechanism. 
%Thus momentum conservation also enforces that plasmon scattering is the only loss mechanism when a constant external potential is applied.

%From these results, we can conclude that the enforcing collisional invariants in the relaxation-time approximation is a crude way to include local field corrections beyond the RPA into the susceptibilty of collisionally damped charged particles.

Our results extend Selchow et al. \cite{Selchow1999} and Atwal and Ashcroft's work from the single-species BGK to a multi-species BGK.
%showing that Haack et al.’s multi-species BGK kinetic equation could produce number, momentum, and energy conserving multi-species susceptibilities.
If we reconsider Selchow et al. \cite{Selchow1999}, which showed that both the Fokker-Plank and BGK kinetic equations both recover the Mermin dielectric response function, then our results raise two questions. First, can the multi-species Fokker-Plank equations recover the multi-species Mermin response? Second, can the Fokker-Plank kinetic equation produce the same momentum and energy conserving susceptibility?
If both questions are answered in the affirmative, then this would suggest that the collisional model's form is less important than the collisional invariants in determining the dynamical response of collisionally damped charged particles. 

We produced the two-component completed Mermin ion-ion DSF and applied the model to a plasma of deuterium and tritium at ICF hot spot conditions. 
Comparing the completed Mermin DSF to the Mermin and RPA DSFs, we showed that conservation of momentum produces a peak near the ion plasma frequency not present in the Mermin and RPA models.
This suggests that ion-phonon scattering is an important energy loss mechanism in the warm dense matter regime. 
We also show that the light species approximation is in qualitative agreement with all mixed or unmixed deuterium or tritium.
Using the light species approximation, we show that carbon contamination affects the Mermin DT DSF in a qualitatively different way than either the RPA and the completed Mermin DSF.
We recommend studying the impact of dynamical inter-species collision frequencies $\tau_{ij}(\omega)$ and effective ion-ion interaction potentials $v_{ij}(k)$ before making direct comparisons to experiments.

Finally, we applied our completed Mermin conductivity model to dynamical gold conductivity measurements. 
We showed the impact of number and momentum conservation on the shape the conductivity fit.
We see that number conservation and moment conservation can both suppress the DC conducitivity, but in different ways.
Therefore, our completed Mermin model extends the Drude-Smith model.
Based on relavent conservation laws, we conclude that the completed Mermin conductivity, \eqref{eq_epsAAk0}, can model back scattering with the parameters set to $a=1$ (number conservation turned on) and $b \in [-1,0]$ (momentum reversed in the collision).

